Closure Conversion, Flat Environments, and the Complexity of Abstract Machines

Closure conversion is a program transformation at work in compilers for functional languages to turn inner functions into global ones, by building closures pairing the transformed functions with the environment of their free variables. Abstract machines rely on similar and yet different concepts of closures and environments. In this paper, we study the relationship between the two approaches. We adopt a very simple {\lambda}-calculus with tuples as source language and study abstract machines for both the source language and the target of closure conversion. Moreover, we focus on the simple case of flat closures/environments, that is, with no sharing of environments. We provide three contributions. Firstly, a new simple proof technique for the correctness of closure conversion, inspired by abstract machines. Secondly, we show how the closure invariants of the target language allow us to design a new way of handling environments in abstract machines, not suffering the shortcomings of other styles. Thirdly, we study the machines from the point of view of time complexity, adapting analyses by Accattoli and co-authors. We show that closure conversion decreases various dynamic costs while increasing the size of the initial code. Despite these changes, the overall complexity of the machines before and after closure conversion turns out to be the same.

==> proofs/01b-source_machine/blue_search_bound.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	Every transition $\tomachseaoneev$ in $\exec$ must be preceded by a transition $\tomachseaonenv$ (otherwise there would not be an entry of shape $\nvsym\clos$ in the stack), thus $\sizep\exec{sea_{1}\evsym}   \leq \sizep\exec{sea_{1}\nvsym}$.
	
	Every transition $\tomachseathreeev$ in $\exec$ must be preceded by a transition $\tomachseathreenv$ (otherwise there would not be an entry of shape $\tuple{\machctxhole,\mydots}$ in the stack), thus $\sizep\exec{sea_{3}\evsym}   \leq \sizep\exec{sea_{3}\nvsym}$.
	
	Every transition $\tomachprojev$ in $\exec$ must be preceded by a transition $\tomachseatwonv$ (otherwise there would not be an entry of shape $\proj_{i}$ in the stack), thus $\sizep\exec{
	\projsym}   \leq \sizep\exec{sea_{2}\nvsym}$.
	\qedhere
\end{proof}


==> proofs/01b-source_machine/final_calculations.tex <==
% !TEX root = ../../main.tex
\begin{proof}
First, we prove $\omeas\state \leq \omeas{\compil\tm} + \sizep\exec{\evsym\betav}\cdot\size\tm-\sizep\exec{\nvsym\subsym,\nvsym sea_{1-5},\evsym sea_{6}}$, and then we deduce the statement. The proof is by induction on the length $\size\exec$ of $\exec$. If $\exec$ is empty then the inequality becomes $\omeas\state= \omeas{\compil\tm} \leq \omeas{\compil\tm}$, which is true. If $\exec$ is non-empty then one considers the last transitions of $\exec$, that is, let $\exectwo:\compil\tm \totam^{\size\exec-1} \statetwo$ be $\exec$ without its last transition $\statetwo \totam \state$. By \ih,  $\omeas\state \leq \omeas{\compil\tm} + \sizep\exectwo{\evsym\betav}\cdot\size\tm-\sizep\exectwo{\nvsym\subsym,\nvsym sea_{1-5},\evsym sea_{6}}$. Case of this last transition:
\begin{itemize}
\item $\tomachbetaev$: by \reflemma{TAM-overhead}.1, the left-hand side of the inequality grows of at most $\size\tm$, which is also the increase of the right-hand side.
\item $\tomachhole{\nvsym\subsym,\nvsym sea_{1-5},\evsym sea_{6}}$: by \reflemma{TAM-overhead}.2, the left-hand side of the inequality decreases of at least $1$, and the right-hand side decreases of 1.
\item $\tomachhole{\evsym\proj,\evsym sea_{1-3}}$: by \reflemma{TAM-overhead}.3, both the left-hand and the right-hand side of the inequality do not change.
\end{itemize}
Thus, we proved the inequality. It follows that $\sizep\exec{\nvsym\subsym,\nvsym sea_{1-5},\evsym sea_{6}} \leq \omeas{\compil\tm} + \sizep\exec{\evsym\betav}\cdot\size\tm$. By definition and \reflemma{TAM-size-vs-overhead}, $\omeas{\compil{\tm}} = \omeas{\nvsym(\tm,\emptyenv)} = \omeas{\tm} \leq_{\reflemmaeq{TAM-size-vs-overhead}} \size\tm$. Then, 
\[\omeas{\compil\tm} + \sizep\exec{\evsym\betav}\cdot\size\tm \ \ \leq \ \ \size\tm + \sizep\exec{\evsym\betav}\cdot\size\tm \ \ =\ \  (\sizep\exec{\evsym\betav}+ 1)\cdot\size\tm.\]
Summing up, the inequality is:
\[\sizep\exec{\nvsym\subsym,\nvsym sea_{1-5},\evsym sea_{6}} \leq (\sizep\exec{\evsym\betav}+ 1)\cdot\size\tm\]
Now, we finally obtain our bound of $\size\exec$ by applying twice the derived inequality:
\begin{center}
$\begin{array}{llll}
	\size{\exec} &= & \sizep\exec{\nvsym\subsym,\nvsym sea_{1-5}} + \sizep\exec{\evsym \beta}+ \sizep\exec{\evsym\proj,\evsym sea_{1,3,6}}
	\\
	&\leq_{\reflemmaeq{TAM-blue-bound}} &\sizep\exec{\nvsym\subsym,\nvsym sea_{1-5}} + \sizep\exec{\evsym \beta}+ \sizep\exec{\nvsym sea_{1-3},\evsym sea_{6}}
	\\
	&\leq & \sizep\exec{\evsym \beta} + 2\cdot(\sizep\exec{\evsym\betav}+ 1)\cdot\size\tm
	\\
	&\leq & 3\cdot(\sizep\exec{\evsym\betav}+ 1)\cdot\size\tm
\end{array}$
\end{center}
Where the last inequality is justified by the fact that $\size{\tm} \geq 1$.
\qedhere
\end{proof}

==> proofs/01b-source_machine/measure_properties.tex <==
% !TEX root = ../../main.tex
\begin{proof}
\hfill
	\begin{enumerate}
		\item \emph{Beta}: $\state = \pairstate{\evsym (\la{\tuvar}\tmtwo,  \env)}{\vv\clos \cons\stack}
		\tomachbeta \pairstate{
			\nvsym (\tmtwo, \esub\tuvar{\vv\clos} \cons \env)} {\stack} = \statetwo$. 
		Then, $\omeas\statetwo \leq \omeas\state + \size{\tm}$ because:
		\begin{align*}
			\omeas{\state} &= \omeas{\stack} 
			& 
			\omeas{\statetwo} &= \omeas{\tmtwo} + \omeas{\stack} \overset{\reflemmaeq{TAM-size-vs-overhead}}{\leq} \size{\tmtwo} + \omeas{\stack} \overset{\reflemmaeq{TAM-sub-term-invariant}}{\leq} \size{\tm} + \omeas{\stack}
		\end{align*}
	
		\item 
		\begin{enumerate}
			\item $\state = \pairstate{\nvsym (\tm\tmtwo, \env)}{\stack }
			\tomachseaonenv
			\pairstate{\nvsym (\tmtwo, \env)} { \nvlab{\pair\tm\env} \cons\stack } =\statetwo$.
			Then, $\omeas{\statetwo} < \omeas{\state}$ because:
			\begin{align*}
				\omeas{\state} &= 1 + \omeas{\tm} + \omeas{\tmtwo} + \omeas{\stack} 
				& 
				\omeas{\statetwo} &= \omeas{\tm} + \omeas{\tmtwo} + \omeas{\stack} 
			\end{align*}
%%%%%%%%%%
			\item $\state=\pairstate{\nvsym (\proj_i \tm , \env) }{ \stack} 
			\tomachseatwonv 
			\pairstate{\nvsym (\tm,\env)}{ \proj_i \cons \stack }=\statetwo$. 
			Then, $\omeas{\statetwo} < \omeas{\state}$ because:
			\begin{align*}
				\omeas{\state} &= 1 + \omeas{\tm} +  \omeas{\stack} 
				& 
				\omeas{\statetwo} &= \omeas{\tm} + \omeas{\stack} 
			\end{align*}
			
%%%%%%%%%%%%%
			\item $\state=\pairstate{\nvsym (\tuple{\mydots,\tm_n}, \env)} {\stack} 
			\tomachseathreenv 
			\pairstate{\nvsym   (\tm_n, \env)  }{\pair{\tuple{\mydots,\machctxhole}}\env \cons \stack}=\statetwo$ with  $ n >0$. 
			Then, $\omeas{\statetwo} < \omeas{\state}$ because:
			\begin{align*}
				\omeas{\state} &= n + \sum_{i=1}^n\omeas{\tm_i} +  \omeas{\stack} 
				& 
				\omeas{\statetwo} &= n-1 +\sum_{i=1}^n\omeas{\tm_i} + \omeas{\stack} 
			\end{align*}
			
%%%%%%%%%%%%%%%%%%%%
			\item $\state=\pairstate{\nvsym (\tuple{}, \env) }{\stack}  \tomachseafournv 
			\pairstate{\evsym (\tuple{}, \emptyenv) } {\stack} =\statetwo$. 
			Then, $\omeas{\statetwo} < \omeas{\state}$ because:
			\begin{align*}
				\omeas{\state} &= 1 +   \omeas{\stack} 
				& 
				\omeas{\statetwo} &= \omeas{\stack} 
			\end{align*}
			
%%%%%%%%%%%%%%%
			\item $\state=\pairstate{\nvsym  (\la\tuvar\tm, \env)} {\stack} 
			\tomachseafivenv 
			\pairstate{\evsym (\la\tuvar\tm , \env)} {\stack }=\statetwo$. 
			Then, $\omeas{\statetwo} < \omeas{\state}$ because:
			\begin{align*}
				\omeas{\state} &= 1 +   \omeas{\stack} 
				& 
				\omeas{\statetwo} &= \omeas{\stack} 
			\end{align*}
			
%%%%%%%%%%%%%%
			\item $\state=\pairstate{\nvsym (\var, \env)} {\stack} 
			\tomachsub
			\pairstate{\env(\var)} {\stack} =\statetwo$.
			Then, $\omeas{\statetwo} < \omeas{\state}$ because $\env(\var) = \clos$ and:
			\begin{align*}
				\omeas{\state} &= 1 +   \omeas{\stack} 
				& 
				\omeas{\statetwo} &= \omeas{\stack} 
			\end{align*}
			
%%%%%%%%%%%%
			\item $\state=\pairstate{\clos} {\pair{\tuple{\mydots,\tm_n,\machctxhole,\mydots}}\env \cons\stack }
			\tomachseasixev
			\pairstate{\nvsym (\tm_n ,\env) }  {\pair{\tuple{\mydots,\tm_{n-1},\machctxhole,\clos,\mydots}}\env \cons\stack }=\statetwo$ with $n > 0$.
			Then, $\omeas{\statetwo} < \omeas{\state}$ because $n > 0$ and:
			\begin{align*}
				\omeas{\state} &= n + \sum_{i=1}^n\omeas{\tm_i} + \omeas{\stack} 
				& 
				\omeas{\statetwo} &= n-1 + \sum_{i=1}^n\omeas{\tm_i} + \omeas{\stack} 
			\end{align*}
		\end{enumerate}
	
		\item 
		\begin{enumerate}
			\item\emph{Projection}: $\pairstate{\vv\clos} {\proj_i \cons \stack}
			\tomachproj 
			\pairstate{\clos_i}{\stack} $ with $i \leq \norm{\vv\clos}$.
			Then, $\omeas{\statetwo} = \omeas{\stack} = \omeas{\state}$.
			\item $\pairstate{\clos}{ \nvlab{\pair\tm\env} \cons\stack} 
			\tomachseaoneev
			\pairstate{\nvsym (\tm,\env)} {\clos \cons\stack}$. 
			Then, $\omeas{\statetwo} = \omeas{\tm} + \omeas{\stack} = \omeas{\state}$.
			\item $\pairstate{\clos}{ \pair{\tuple{\machctxhole,\mydots}}\env \cons\stack} 
			\tomachseathreeev
			\pairstate{\tuple{\clos,\mydots}} {\stack} $. 
			Then, $\omeas{\statetwo} = \omeas{\stack} = \omeas{\state}$.\qedhere
		\end{enumerate}

	\end{enumerate}
\end{proof}

==> proofs/01b-source_machine/sub-term_invariant.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on the length $\length{\exec}$ of the execution $\exec \colon \compil{\tm} \totam^{*} \state$. 
	If $\length{\exec} = 0$ then the statement trivially holds, since $\state = \compil{\tm} = (\tm, \emptyenv,\emptyenv,\emptyenv)$.
	
	Otherwise $\exec \colon \compil{\tm} \totam^{*} \state$ is the concatenation of $\exectwo \colon \compil{\tm} \totam^{*} \statetwo$ and $\statetwo \totam \state$.
	By \ih, the statement holds for $\exectwo$. A straightforward analysis of the transition rules of the machine proves that the statement is preserved by the transition $\statetwo \totam \state$.
	\qedhere
\end{proof}


==> proofs/01c-source_complexity/TAM_complexity.tex <==
% !TEX root = ../../main.tex
\begin{proof}
\ben{bla}.
\qedhere
\end{proof}

==> proofs/01c-source_complexity/cost_of_transitions.tex <==
% !TEX root = ../../main.tex
\begin{proof}
\ben{bla}.
\qedhere
\end{proof}

==> proofs/02a-intermediate_calculus/implementation_source_intermediate.tex <==
%!TEX root = ../../main.tex
\begin{proof}
\hfill
\begin{enumerate}
\item By induction on $k$. For $k=0$ the statement holds because $\unlali{\lali\tm} = \tm$ by the inverse property of the reverse translation (\reflemma{rev-transl-properties}.1). For $k>0$, let the sequence be $\tm \tosou^{k-1} \tmthree \tosou \tmtwo$. By \ih, $\lali\tm \toint^{k-1} \tmthree'$ with $\unlali{\tmthree'}=\tmthree$ and with steps as in the statement. Note that if $\tmthree'$ is $\toint$-normal then, by the halt property of the reverse translation (\refprop{rev-transl-implem-bricks}.2, which can be applied because the closure hypothesis is preserved by reduction, so that $\tmthree'$ is closed), then $\tmthree$ is $\tosou$-normal, against hypotheses. Then $\tmthree' \toint \tmtwo'$. By projection (\refprop{rev-transl-implem-bricks}.1), $\unlali{\tmthree'} =\tmthree \tosou \unlali{\tmtwo'}$ and it is the same kind of step than on $\intcal$. Since $\tosou$ is deterministic (\reflemma{source-determinism}), $\unlali{\tmtwo'}=\tmtwo$. 

Now, if $\tmtwo$ is a value assume by contradiction that $\tmtwo'$ is not a value. By harmony of $\intcal$ (\reflemma{intermediate-harmony}), $\tmtwo'$ reduces and by projection $\tmtwo$ reduces, which implies that $\tmtwo$ is not a value by harmony of $\soucal$ (\reflemma{source-harmony}). Absurd.
%%%
\item By induction on $k$. For $k=0$ the statement holds because $\unlali{(\lali\tm)} = \tm$ by the inverse property of the reverse translation (\reflemma{rev-transl-properties}.1). For $k>0$, let the sequence be $\lali\tm \toint^{k-1} \tmthree \toint \tmtwo$. By \ih, $\tm \tosou^{k-1} \unlali\tmthree$ and with steps as in the statement. By the projection of $\toint$ steps via the reverse translation (\refprop{rev-transl-implem-bricks}.1), $\unlali\tmthree \tosou \unlali\tmtwo$ and it is the same kind of step than on $\intcal$. The \emph{moreover} part follows from \reflemma{rev-transl-properties}.2.\qedhere
\end{enumerate}
\end{proof}

==> proofs/02b-intermediate_machine/closed_values_invariant.tex <==
% !TEX root = ../../main.tex
\begin{proof}
By induction on the length of the execution ending on $\state$. For each transition, it immediately follows from the \ih, but for $\tomachsubwev$ which needs the well-formed invariant (\reflemma{LTAM-wabs-invariant}) to prove that $\evsym  \pack{ \dabsv\vartwo\var\nvsym\tm}{\evlab\val}$ is closed.\qedhere
\end{proof}


==> proofs/02b-intermediate_machine/closure_invariant.tex <==
% !TEX root = ../../main.tex
\begin{proof}
The two parts: 
	\begin{enumerate}
		\item[a] $\fv\tm \cup \fv\stack\subseteq \dom\env$;
		\item[b] $\fv\stacktwo\subseteq \dom\envtwo$ for every entry $\pair\stacktwo\envtwo$ of the environment stack $\ars$.
	\end{enumerate}
are proved at the same time, by induction on the length of the execution ending on $\state$. For most transitions, it immediately follows from the \ih The relevant cases are (they show in particular that the two parts have to be proved simultaneously):
\begin{enumerate}
\item In $\tomachsubwev$ and $\tomachsubvev$, we need the closed values invariant (Point 2) on the source state to prove part $a$ about $\env(\var)$ for the target state.
\item In $\tomachseasevenev$, we need part $b$ and the closed values invariant (Point 2) on the source state to prove part $a$ for the target state.
\item In $\tomachbetaev$, we need part $a$ on the source state to prove part $b$ on the target state. Part $a$ for the target state holds because of the well-formed invariant (Point 1).\qedhere
\end{enumerate}
\end{proof}


==> proofs/02b-intermediate_machine/well_abstracted_invariant.tex <==
% !TEX root = ../../main.tex
\begin{proof}
By induction on the length of the execution ending on $\state$. For the initial state, it follows from the requirement that compiled terms are prime (which is an extension of well-formed). For the inductive case, one considers each transition, and the statement for the target state immediately follows from the \ih about the source state.\qedhere
\end{proof}


==> proofs/02c-int_complexity/LTAM_complexity.tex <==
% !TEX root = ../../main.tex
\begin{proof}
\ben{bla}.
\qedhere
\end{proof}

==> proofs/02c-int_complexity/cost_of_transitions.tex <==
% !TEX root = ../../main.tex
\begin{proof}
\ben{bla}.
\qedhere
\end{proof}

==> proofs/03a-target_calculus/implementation_intermediate_target.tex <==
%!TEX root = ../../main.tex
\begin{proof}
\hfill
\begin{enumerate}
\item By induction on $k$. For $k=0$ the statement trivially holds. For $k>0$, let the sequence be $\tm \toint^{k-1} \tmthree \toint \tmtwo$. By \ih, $\clc\tm\vartwolist\varlist \totar^{k-1} \clc\tmthree\vartwolist\varlist$ and with steps as in the statement. By projection (\refprop{rev-transl-implem-bricks}.1), $\clc\tmthree\vartwolist\varlist  \totar \clc\tmtwo\vartwolist\varlist$ and it is the same kind of step as in $\intcal$. The \emph{moreover} part follows from \reflemma{varelim-properties}.1.
%%%
\item By induction on $k$. For $k=0$ the statement trivially holds. For $k>0$, let the sequence be $\clc\tm\vartwolist\varlist \totar^{k-1} \tmtwo \totar \tmthree$. By \ih, $\tm\toint^k\tmtwo'$ and $\clc{\tmtwo'}\vartwolist\varlist=\tmtwo$, with steps as in the statement. By the halt property of name elimination (\refprop{tar-simulation}.2), $\tmtwo'$ cannot be $\toint$-normal, otherwise $\tmtwo$ would be $\totar$-normal. Then $\tmtwo'\toint\tmthree'$ for some $\tmthree'\in\intcal$. By projection of $\toint$ steps via name elimination (\refprop{tar-simulation}.1), $\tmtwo = \clc{\tmtwo'}\vartwolist\varlist \totar \clc{\tmthree'}\vartwolist\varlist$ and it is the same kind of step as in $\intcal$. Since $\totar$ is deterministic (\reflemma{target-determinism}), $\clc{\tmthree'}\vartwolist\varlist=\tmthree$.

Now, if $\tmtwo$ is $\totar$-normal assume by contradiction that $\tmthree$ is not $\toint$-normal. Then it reduces, and by projection $\tmtwo$ reduces---absurd. So, $\tmthree$ is $\toint$ normal. By the halt property, $\tmthree$ is a value, otherwise it would be a clash, and $\tmtwo$ would also be a clash.
\qedhere
\end{enumerate}
\end{proof}

==> proofs/03a-target_calculus/implementation_source_target.tex <==
%!TEX root = ../../main.tex
\begin{proof}
\hfill
\begin{enumerate} 

\item Since $\tm$ is closed, we have $\fv\tm\subseteq\emptylist\vdisjoint\emptylist$. By the $\soucal/\intcal$ implementation theorem (\refthm{sou-int-implementation}), there exists $\derivtwo:\lali\tm \toint^{k} \tmthree$ with $\unlali{\tmthree}=\tmtwo$. By the $\intcal/\tarcal$ implementation theorem (\refthm{int-tar-implementation}), there exists $\derivthree:\clc{\lali\tm}\emptylist\emptylist \totar^{k} \clc{\tmthree}\emptylist\emptylist$. Set $\tmtwo\defeq \clc{\tmthree}\emptylist\emptylist$. By the inverse property of the naming translation (\refprop{tar-rev-transl-inverse}), $\namingp\tmtwo\emptylist\emptylist = \namingp{\clc{\tmthree}\emptylist\emptylist}\emptylist\emptylist =\tmthree$. Therefore, $\unlali{\namingp\tmtwo\emptylist\emptylist} = \unlali\tmthree=\tmtwo$.

It follows by composing the \emph{moreover} parts of the two theorems.

%%%
\item By the $\intcal/\tarcal$ implementation theorem (\refthm{int-tar-implementation}), there exists $\derivthree:\lali\tm\toint^{k} \tmthree$ such that $\clc\tmthree\emptylist\emptylist=\tmtwo$. By the inverse property of the naming translation (\refprop{tar-rev-transl-inverse}), $\namingp\tmtwo\emptylist\emptylist = \namingp{\clc{\tmthree}\emptylist\emptylist}\emptylist\emptylist =\tmthree$. By the $\soucal/\intcal$ implementation theorem (\refthm{sou-int-implementation}), there exists $\derivtwo:\tm \toint^{k} \unlali\tmthree = \unlali{\namingp\tmtwo\emptylist\emptylist}$. It follows by composing the \emph{moreover} parts of the two theorems.
\qedhere
\end{enumerate}
\end{proof}
